Conformal Prediction with Temporal Quantile Adjustments

We develop Temporal Quantile Adjustment (TQA), a general method to construct efficient and valid prediction intervals (PIs) for regression on cross-sectional time series data. Such data is common in many domains, including econometrics and healthcare. A canonical example in healthcare is predicting patient outcomes using physiological time-series data, where a population of patients composes a cross-section. Reliable PI estimators in this setting must address two distinct notions of coverage: cross-sectional coverage across a cross-sectional slice, and longitudinal coverage along the temporal dimension for each time series. Recent works have explored adapting Conformal Prediction (CP) to obtain PIs in the time series context. However, none handles both notions of coverage simultaneously. CP methods typically query a pre-specified quantile from the distribution of nonconformity scores on a calibration set. TQA adjusts the quantile to query in CP at each time $t$, accounting for both cross-sectional and longitudinal coverage in a theoretically-grounded manner. The post-hoc nature of TQA facilitates its use as a general wrapper around any time series regression model. We validate TQA's performance through extensive experimentation: TQA generally obtains efficient PIs and improves longitudinal coverage while preserving cross-sectional coverage.

==> figure_and_table.tex <==


\def \FigResid{
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/NeurIPS_residual.png}
    %\vskip\baselineskip
\caption
{
Sorted absolute residuals ($|y-\hat{y}|$) with x-axis denoting the percentile and y-axis denoting the scale of residual for $t=T-10$. 
Each dataset is normalized such that the mean of the residuals is 1.
To cover the extreme values, even if allowed to ``sacrifice'' some less extreme values, the PI on average is expected to get much wider.
It is thus surprising that \methodBudget could improve \textit{both} efficiency and the coverage for extreme TS.
\label{fig:exp:resid}
}
\end{figure}
}


\def \FigTailCoverage{
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/NeurIPS_TCR_CLAIM.png}%
    \includegraphics[width=0.5\textwidth]{Figures/NeurIPS_TCR_GEFComR.png}
    %\vskip\baselineskip
\caption
{
Coverage rate (Y-axis) vs the percentile among all test TS (X-axis, with zero meaning the least-covered TS) for the 10\% least-covered TS in CLAIM (left) and GEFCom-R (right).
%We show the coverage rate for the 10\% least-covered time-series for CLAIM (left) and GEFCom-R (right). 
%The Y-axis is the average coverage rate, and the X-axis is the percentile among all test time-series (zero means the least-covered time-series).
The bands denote the center 80\% realizations.
\methodError has an natural advantage over \methodBudget by using infinitely-wide PI.
However, even \methodBudget still significantly improves the longitudinal coverage rate over all baselines.
\label{fig:exp:tail}
}
\end{figure}
}

\def\TabTCRScaled{
\begin{table}[ht]
%===============Begin of Table====================
\captionof{table}{
The tail coverage rate (mean coverage rate for the least-covered 10\% time-series), \textit{after re-scaling the PI widths such that all methods have the same mean width as CFRNN.}
%Minimum and the 25-th percentile (across time-series) of average coverage rates.
%This measures the worst/worse case scenario.
We want the tail coverage rate to be as high as possible.
The best method is in \textbf{bold}.
%\fontred{Find a way to show that without re-scaling, \methodError is good.}
%\fontred{This might be better shown with (violin) plots.}
\methodBudget consistently outperforms baselines, except on the MIMIC dataset.
\methodError is excluded from this table because of the existence of infinitely-wide PIs.
}
\begin{center}
\begin{scriptsize}
\setlength\tabcolsep{6pt}
\begin{tabular}{l|c|ccc|cr}
\toprule
Tail Coverage Rate  & \methodBudget & CFRNN (Split) & CQRNN & LASplit &  QRNN  & DPRNN  \\
\midrule
MIMIC & 70.90$\pm$3.29  & 62.22$\pm$7.09 & \textbf{74.57$\pm$3.59} & 62.18$\pm$6.07 & 74.09$\pm$3.45 & 66.70$\pm$6.25\\
CLAIM & \textbf{73.66$\pm$1.17} & 65.95$\pm$1.88 & 68.73$\pm$3.02 & 68.01$\pm$2.44 & 65.18$\pm$3.16 & 47.09$\pm$3.41\\
COVID & \textbf{70.01$\pm$4.22} & 63.89$\pm$6.35 & 61.34$\pm$6.03 & 67.44$\pm$4.80 & 61.92$\pm$5.93 & 53.40$\pm$5.89\\
EEG & \textbf{61.48$\pm$0.67} & 41.75$\pm$1.02 & 41.19$\pm$1.04 & 41.75$\pm$1.02 & 41.44$\pm$1.55 & 18.14$\pm$7.11\\
GEFCom & \textbf{68.83$\pm$0.94} & 58.49$\pm$1.38 & 59.24$\pm$1.52 & 59.48$\pm$1.67 & 59.51$\pm$2.45 & 29.52$\pm$2.03\\
GRFCom-R & \textbf{74.94$\pm$1.05}  & 68.76$\pm$2.18 & 69.38$\pm$1.56 & 69.95$\pm$2.07 & 69.32$\pm$1.87 & 31.48$\pm$1.84\\
\bottomrule
\end{tabular}
\label{table:exp:real:tcr_scaled}
\end{scriptsize}
\end{center}
%===============End of Table====================
\end{table}
}
%\TabTCRScaled




\def\TabAppendixWidthFullTS{

\begin{table}[ht]
%===============Begin of Table====================
\captionof{table}{
Meidan and mean width of the PIs (full TS)
}
\begin{center}
\begin{scriptsize}
\setlength\tabcolsep{6pt}
\begin{tabular}{l|cc|ccc|cr}
\toprule
Median Width $\downarrow$ & \\%TQA-B & TQA-E & CFRNN & CQRNN & LASplit & QRNN & DPRNN\\
\midrule
MIMIC & 1.778$\pm$0.149 & 1.734$\pm$0.124 & 1.788$\pm$0.153 & \textbf{1.528$\pm$0.129} & 1.667$\pm$0.156 & 1.299$\pm$0.114 & 0.484$\pm$0.021\\
CLAIM & 2.679$\pm$0.045 & 2.624$\pm$0.045 & 2.718$\pm$0.049 & 2.669$\pm$0.040 & \textbf{2.472$\pm$0.044} & 2.396$\pm$0.028 & 0.437$\pm$0.017\\
COVID & 0.721$\pm$0.031 & \textbf{0.693$\pm$0.028} & 0.721$\pm$0.032 & 0.739$\pm$0.056 & \textbf{0.684$\pm$0.030} & 0.720$\pm$0.065 & 0.358$\pm$0.028\\
EEG & 5.840$\pm$0.064 & \textbf{4.844$\pm$0.031} & 5.933$\pm$0.071 & 5.936$\pm$0.069 & 5.934$\pm$0.070 & 5.929$\pm$0.084 & 0.135$\pm$0.017\\
GEFCom & 0.186$\pm$0.004 & 0.181$\pm$0.003 & 0.184$\pm$0.004 & 0.188$\pm$0.004 & \textbf{0.177$\pm$0.004} & 0.143$\pm$0.005 & 0.439$\pm$0.007\\
GEFCom-R & 0.160$\pm$0.007 & 0.158$\pm$0.005 & 0.159$\pm$0.007 & 0.157$\pm$0.004 & \textbf{0.151$\pm$0.005} & 0.137$\pm$0.004 & 0.473$\pm$0.009\\
\midrule
Mean Width $\downarrow$ & \\% TQA-B & TQA-E & CFRNN & CQRNN & LASplit & QRNN & DPRNN\\
\midrule
MIMIC & 1.871$\pm$0.148 & 2.273$\pm$0.300 & 1.818$\pm$0.146 & \textbf{1.649$\pm$0.139} & 1.908$\pm$0.174 & 1.422$\pm$0.128 & 0.568$\pm$0.028\\
CLAIM & 2.765$\pm$0.039 & 2.965$\pm$0.056 & 2.721$\pm$0.046 & \textbf{2.643$\pm$0.042} & 2.725$\pm$0.051 & 2.367$\pm$0.028 & 0.567$\pm$0.031\\
COVID & \textbf{0.738$\pm$0.031} & 1.006$\pm$0.223 & \textbf{0.729$\pm$0.034} & 0.780$\pm$0.067 & \textbf{0.728$\pm$0.037} & 0.755$\pm$0.069 & 0.472$\pm$0.039\\
EEG & 5.447$\pm$0.044 & 5.769$\pm$0.061 & \textbf{5.376$\pm$0.041} & \textbf{5.392$\pm$0.041} & \textbf{5.377$\pm$0.041} & \textbf{5.391$\pm$0.060} & 0.177$\pm$0.015\\
GEFCom & 0.198$\pm$0.004 & 0.233$\pm$0.010 & \textbf{0.193$\pm$0.004} & 0.201$\pm$0.004 & 0.197$\pm$0.004 & 0.157$\pm$0.005 & 0.559$\pm$0.008\\
GEFCom-R & 0.167$\pm$0.004 & 0.184$\pm$0.008 & \textbf{0.164$\pm$0.004} & 0.172$\pm$0.004 & 0.167$\pm$0.004 & 0.153$\pm$0.004 & 0.542$\pm$0.010\\
\bottomrule
\end{tabular}
\label{table:exp:appendix:width_full}
\end{scriptsize}
\end{center}
%===============End of Table====================
\end{table}
}
